On the Generalization of Diffusion Model

The diffusion probabilistic generative models are widely used to generate high-quality data. Though they can synthetic data that does not exist in the training set, the rationale behind such generalization is still unexplored. In this paper, we formally define the generalization of the generative model, which is measured by the mutual information between the generated data and the training set. The definition originates from the intuition that the model which generates data with less correlation to the training set exhibits better generalization ability. Meanwhile, we show that for the empirical optimal diffusion model, the data generated by a deterministic sampler are all highly related to the training set, thus poor generalization. This result contradicts the observation of the trained diffusion model's (approximating empirical optima) extrapolation ability (generating unseen data). To understand this contradiction, we empirically verify the difference between the sufficiently trained diffusion model and the empirical optima. We found, though obtained through sufficient training, there still exists a slight difference between them, which is critical to making the diffusion model generalizable. Moreover, we propose another training objective whose empirical optimal solution has no potential generalization problem. We empirically show that the proposed training objective returns a similar model to the original one, which further verifies the generalization ability of the trained diffusion model.

==> reference.tex <==
@article{perkowski2011backward,
	title={Backward stochastic differential equations: an introduction},
	author={Perkowski, Nicolas},
	journal={Tan{\'a}ri jegyzet},
	pages={8},
	year={2011}
}

@inproceedings{kingma2013auto,
	title={Auto-encoding variational $\{$Bayes$\}$},
	author={Kingma, Diederik P and Welling, Max},
	booktitle={International Conference on Learning Representations},
	year={2013}
}

@inproceedings{goodfellow2014generative,
	title={Generative Adversarial Nets},
	author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron C and Bengio, Yoshua},
	booktitle={Advances in Neural Information Processing Systems},
	year={2014}
}

@inproceedings{song2020score,
	title={Score-Based Generative Modeling through Stochastic Differential Equations},
	author={Song, Yang and Sohl-Dickstein, Jascha and Kingma, Diederik P and Kumar, Abhishek and Ermon, Stefano and Poole, Ben},
	booktitle={International Conference on Learning Representations},
	year={2020}
}

@inproceedings{ho2020denoising,
	title={Denoising diffusion probabilistic models},
	author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
	booktitle={Advances in Neural Information Processing Systems},
	year={2020}
}

@inproceedings{arora2017generalization,
	title={Generalization and equilibrium in generative adversarial nets (gans)},
	author={Arora, Sanjeev and Ge, Rong and Liang, Yingyu and Ma, Tengyu and Zhang, Yi},
	booktitle={International Conference on Machine Learning},
	year={2017}
}

@inproceedings{arjovsky2017wasserstein,
	title={Wasserstein generative adversarial networks},
	author={Arjovsky, Martin and Chintala, Soumith and Bottou, L{\'e}on},
	booktitle={International conference on machine learning},
	year={2017}
}

@techreport{somepalli2022diffusion,
	title={Diffusion Art or Digital Forgery? Investigating Data Replication in Diffusion Models},
	author={Somepalli, Gowthami and Singla, Vasu and Goldblum, Micah and Geiping, Jonas and Goldstein, Tom},
	type={Preprint},
	number={arXiv:2212.03860},
	year={2022}
}

@inproceedings{song2020denoising,
	title={Denoising Diffusion Implicit Models},
	author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
	booktitle={International Conference on Learning Representations},
	year={2022}
}

@inproceedings{lu2022dpm,
	title={DPM-Solver: A Fast ODE Solver for Diffusion Probabilistic Model Sampling in Around 10 Steps},
	author={Lu, Cheng and Zhou, Yuhao and Bao, Fan and Chen, Jianfei and Li, Chongxuan and Zhu, Jun},
	booktitle={Advances in Neural Information Processing Systems},
	year={2022}
}

@inproceedings{sohl2015deep,
	title={Deep unsupervised learning using nonequilibrium thermodynamics},
	author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
	booktitle={International Conference on Machine Learning},
	year={2015}
}

@inproceedings{song2021maximum,
	title={Maximum likelihood training of score-based diffusion models},
	author={Song, Yang and Durkan, Conor and Murray, Iain and Ermon, Stefano},
	journal={Advances in Neural Information Processing Systems},
	year={2021}
}

@inproceedings{xu2017information,
	title={Information-theoretic analysis of generalization capability of learning algorithms},
	author={Xu, Aolin and Raginsky, Maxim},
	journal={Advances in Neural Information Processing Systems},
	year={2017}
}

@inproceedings{rodriguez2021tighter,
	title={Tighter expected generalization error bounds via Wasserstein distance},
	author={Rodr{\'\i}guez G{\'a}lvez, Borja and Bassi, Germ{\'a}n and Thobaben, Ragnar and Skoglund, Mikael},
	journal={Advances in Neural Information Processing Systems},
	year={2021}
}

@article{duchi2016lecture,
	title={Lecture notes for statistics 311/electrical engineering 377},
	author={Duchi, John},
	journal={URL: https://stanford. edu/class/stats311/Lectures/full\_notes. pdf. Last visited on},
	volume={2},
	pages={23},
	year={2016}
}

@inproceedings{bao2022analytic,
	title={Analytic-DPM: an Analytic Estimate of the Optimal Reverse Variance in Diffusion Probabilistic Models},
	author={Bao, Fan and Li, Chongxuan and Zhu, Jun and Zhang, Bo},
	booktitle={International Conference on Learning Representations},
	year={2022}
}

@article{banerjee2005optimality,
	title={On the optimality of conditional expectation as a Bregman predictor},
	author={Banerjee, Arindam and Guo, Xin and Wang, Hui},
	journal={IEEE Transactions on Information Theory},
	volume={51},
	number={7},
	pages={2664--2669},
	year={2005},
	publisher={IEEE}
}

@book{wainwright2019high,
	title={High-dimensional statistics: A non-asymptotic viewpoint},
	author={Wainwright, Martin J},
	volume={48},
	year={2019},
	publisher={Cambridge university press}
}

@book{shiryaev2016probability,
	title={Probability-1},
	author={Shiryaev, Albert N},
	volume={95},
	year={2016},
	publisher={Springer}
}

@article{efron2011tweedie,
	title={Tweedie’s formula and selection bias},
	author={Efron, Bradley},
	journal={Journal of the American Statistical Association},
	volume={106},
	number={496},
	pages={1602--1614},
	year={2011},
	publisher={Taylor \& Francis}
}

@article{vincent2011connection,
	title={A connection between score matching and denoising autoencoders},
	author={Vincent, Pascal},
	journal={Neural computation},
	volume={23},
	number={7},
	pages={1661--1674},
	year={2011},
	publisher={MIT Press}
}

@techreport{carlini2023extracting,
	title={Extracting training data from diffusion models},
	author={Carlini, Nicholas and Hayes, Jamie and Nasr, Milad and Jagielski, Matthew and Sehwag, Vikash and Tramer, Florian and Balle, Borja and Ippolito, Daphne and Wallace, Eric},
	type={Preprint},
	number={arXiv:2301.13188},
	year={2023}
}

@inproceedings{allen2019convergence,
	title={A convergence theory for deep learning via over-parameterization},
	author={Allen-Zhu, Zeyuan and Li, Yuanzhi and Song, Zhao},
	booktitle={International Conference on Machine Learning},
	year={2019},
}

@inproceedings{du2019gradient,
	title={Gradient descent finds global minima of deep neural networks},
	author={Du, Simon and Lee, Jason D. and Li, Haochuan and Wang, Liwei and Zhai, Xiyu},
	booktitle={International Conference on Machine Learning},
	year={2019}
}

@article{zhang2021understanding,
	title={Understanding deep learning (still) requires rethinking generalization},
	author={Zhang, Chiyuan and Bengio, Samy and Hardt, Moritz and Recht, Benjamin and Vinyals, Oriol},
	journal={Communications of the ACM},
	volume={64},
	number={3},
	pages={107--115},
	year={2021},
	publisher={ACM New York, NY, USA}
}

@book{vapnik1999nature,
	title={The nature of statistical learning theory},
	author={Vapnik, Vladimir},
	year={1999},
	publisher={Springer science \& business media}
}

@article{yi2022characterization,
	title={Characterization of Excess Risk for Locally Strongly Convex Population Risk},
	author={Yi, Mingyang and Wang, Ruoyu and Ma, Zhi-Ming},
	journal={Advances in Neural Information Processing Systems},
	year={2022}
}

@inproceedings{yi2023breaking,
	title={Breaking Correlation Shift via Conditional Invariant Regularizer},
	author={Yi, Mingyang and Wang, Ruoyu and Sun, Jiacheng and Li, Zhenguo and Ma, Zhi-Ming},
	booktitle={The International Conference on Learning Representations},
	year={2023}
}

@article{bu2020tightening,
	title={Tightening mutual information-based bounds on generalization error},
	author={Bu, Yuheng and Zou, Shaofeng and Veeravalli, Venugopal V},
	journal={IEEE Journal on Selected Areas in Information Theory},
	volume={1},
	number={1},
	pages={121--130},
	year={2020},
	publisher={IEEE}
}

@inproceedings{lopez2018generalization,
	title={Generalization error bounds using Wasserstein distances},
	author={Lopez, Adrian Tovar and Jog, Varun},
	booktitle={2018 IEEE Information Theory Workshop (ITW)},
	pages={1--5},
	year={2018},
	organization={IEEE}
}

@techreport{cao2022survey,
	title={A survey on generative diffusion model},
	author={Cao, Hanqun and Tan, Cheng and Gao, Zhangyang and Chen, Guangyong and Heng, Pheng-Ann and Li, Stan Z},
	journal={Preprint},
	number={arXiv:2209.02646},
	year={2022}
}

@inproceedings{gu2022vector,
	title={Vector quantized diffusion model for text-to-image synthesis},
	author={Gu, Shuyang and Chen, Dong and Bao, Jianmin and Wen, Fang and Zhang, Bo and Chen, Dongdong and Yuan, Lu and Guo, Baining},
	booktitle={Conference on Computer Vision and Pattern Recognition},
	year={2022}
}

@book{wainwright2019,
	author={Wainwright, Martin J.},  
	year= {2019}, 
	series={Cambridge Series in Statistical and Probabilistic Mathematics},
	title={High-dimensional statistics: A non-asymptotic viewpoint},
	publisher={Cambridge University Press}
}

@book{van1996weak,
	title={Weak convergence},
	author={Van Der Vaart, Aad W and Wellner, Jon A and van der Vaart, Aad W and Wellner, Jon A},
	year={1996},
	publisher={Springer}
}

@inproceedings{ronneberger2015u,
	title={U-net: Convolutional networks for biomedical image segmentation},
	author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
	booktitle={Medical Image Computing and Computer-Assisted Intervention--MICCAI 2015: 18th International Conference, Munich, Germany, October 5-9, 2015, Proceedings, Part III 18},
	pages={234--241},
	year={2015},
	organization={Springer}
}

@article{krizhevsky2009learning,
	title={Learning multiple layers of features from tiny images},
	author={Krizhevsky, Alex and Hinton, Geoffrey},
	year={2009},
	publisher={Citeseer}
}

@inproceedings{nichol2021improved,
	title={Improved denoising diffusion probabilistic models},
	author={Nichol, Alexander Quinn and Dhariwal, Prafulla},
	booktitle={International Conference on Machine Learning},
	year={2021}
}

@inproceedings{liu2015deep,
	title={Deep learning face attributes in the wild},
	author={Liu, Ziwei and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
	booktitle={International Conference on Computer Vision},
	year={2015}
}

@inproceedings{deng2009imagenet,
	title={Imagenet: A large-scale hierarchical image database},
	author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
	booktitle={Conference on Computer Vision and Pattern Recognition},
	year={2009}
}

@inproceedings{heusel2017gans,
	title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
	author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
	journal={Advances in Neural Information Processing Systems},
	year={2017}
}

